Assessing the ability of generative adversarial networks to learn canonical medical image statistics

In recent years, generative adversarial networks (GANs) have gained tremendous popularity for potential applications in medical imaging, such as medical image synthesis, restoration, reconstruction, translation, as well as objective image quality assessment. Despite the impressive progress in generating high-resolution, perceptually realistic images, it is not clear if modern GANs reliably learn the statistics that are meaningful to a downstream medical imaging application. In this work, the ability of a state-of-the-art GAN to learn the statistics of canonical stochastic image models (SIMs) that are relevant to objective assessment of image quality is investigated. It is shown that although the employed GAN successfully learned several basic first- and second-order statistics of the specific medical SIMs under consideration and generated images with high perceptual quality, it failed to correctly learn several per-image statistics pertinent to the these SIMs, highlighting the urgent need to assess medical image GANs in terms of objective measures of image quality.

==> images/tab_attenuation_values.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[!t]
\centering
\caption{Linear attenuation coefficients ($\mu$) in cm$^{-1}$ for different tissue types for X-rays of energy 20 keV. Some of the linear attenuation coefficients are obtained directly from the cited references, whereas others are obtained using the density $\rho$ and the mass attenuation coefficients $\mu/rho$ obtained from the linked references. 
% The terminal duct lobular unit (TDLU) and the ducts are categorized as fiberous tissue \cite{}, hence the corresponding $\mu$ values are used. Ligament and skin are categorized as soft tissue \cite{}.
}
\label{tab:attenuation_values}
\begin{tabular}{@{}cc@{}}
\toprule
Tissue type     & Linear attenuation coefficient $\mu$ (cm$^{-1}$)        \\
\midrule
Air             & 0.00093348 \cite{nist}    \\ 
Fat             & 0.488 \cite{chen} \\
Skin            & 0.89707 \cite{nist} \\
Glandular       & 0.783 \cite{tomal}\\
Muscle          & 0.861525 \cite{nist}\\
Ligament        & 0.92176 \cite{nist}\\
TDLU            & 0.918 \cite{chen} \\
Duct            & 0.918 \cite{chen} \\
Artery and Vein & 0.8428 \cite{nist}\\
\bottomrule
\end{tabular}
\end{table}
